I Bet You Are Wrong: Gambling Adversarial Networks for Structured Semantic Segmentation

Adversarial training has been recently employed for realizing structured semantic segmentation, in which the aim is to preserve higher-level scene structural consistencies in dense predictions. However, as we show, value-based discrimination between the predictions from the segmentation network and ground-truth annotations can hinder the training process from learning to improve structural qualities as well as disabling the network from properly expressing uncertainties. In this paper, we rethink adversarial training for semantic segmentation and propose to formulate the fake/real discrimination framework with a correct/incorrect training objective. More specifically, we replace the discriminator with a "gambler" network that learns to spot and distribute its budget in areas where the predictions are clearly wrong, while the segmenter network tries to leave no clear clues for the gambler where to bet. Empirical evaluation on two road-scene semantic segmentation tasks shows that not only does the proposed method re-enable expressing uncertainties, it also improves pixel-wise and structure-based metrics.

==> Gambling Adversarial Networks/Figures/overview_figure.tex <==


\tikzstyle{block} = [draw, rectangle, 
    minimum height=2em, minimum width=4em, node distance=2cm]
\tikzstyle{sum} = [draw, circle, minimum size=1cm, node distance=2cm]
\tikzstyle{dia} = [diamond, draw, text badly centered, inner sep=2t]
\tikzstyle{square} = [draw, rectangle, 
    minimum height=2em, minimum width=2em, node distance=2cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\begin{figure*}[!t]
\centering
\begin{tikzpicture}[auto, node distance=1.4cm,>=latex']
    % We start by placing the blocks
    % \node [input, name=input] {};
    \node[inner sep=0pt, name=x, label={[yshift=-0cm]$x$}](x) {\includegraphics[height=1.2cm ]{Figures/27_rgb.png}};
    \node[draw, rectangle, minimum height=1.2cm, minimum width = 0.05cm, right = 0.2cm of x, name=enc1]{};


    \node[draw, rectangle, node distance=0.4cm, minimum height=1.0cm, minimum width = 0.01cm, right of=enc1, name=enc2]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=0.75cm, minimum width = 0.01cm, right of=enc2, name=enc3]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=0.5cm, minimum width = 0.01cm, right of=enc3, name=enc4, label={[label distance=0.4cm]segmenter ($s$)}]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=0.75cm, minimum width = 0.01cm, right of=enc4, name=dec1]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=1.0cm, minimum width = 0.01cm, right of=dec1, name=dec2]{};
    \node[draw, rectangle, node distance=0.4cm and 1cm, minimum height=1.2cm, minimum width = 0.01cm, right of=dec2, name=dec3]{};
    \node[inner sep=0pt, name=pred, right= 0.2 cm of dec3,  label={[yshift=-0cm]$\hat{y}$}](pred) {\includegraphics[height=1.2cm ]{Figures/27_seg.png}};
    \node[draw, rectangle, minimum height=1.2cm, minimum width = 0.05cm,  right = 0.2 cm of pred, name=enc2_1]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=1.0cm, minimum width = 0.01cm, right of=enc2_1, name=enc2_2]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=0.75cm, minimum width = 0.01cm, right of=enc2_2, name=enc2_3]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=0.5cm, minimum width = 0.01cm, right of=enc2_3, name=enc2_4, label={[label distance=0.4cm]gambler ($g$)}]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=0.75cm, minimum width = 0.01cm, right of=enc2_4, name=dec2_1]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=1.0cm, minimum width = 0.01cm, right of=dec2_1, name=dec2_2]{};
    \node[draw, rectangle, node distance=0.4cm, minimum height=1.2cm, minimum width = 0.01cm, right of=dec2_2, name=dec2_3]{};
    \node[inner sep=0pt, name=bet_map, right = 0.3cm of dec2_3,  label={[yshift=-0cm]$\hat{b}$}](bet_map) {\includegraphics[height=1.2cm ]{Figures/27_betmap.png}};
    \node[inner sep=0pt, name=gt, below = 0.8 cm of  pred, label={[yshift=-0cm]$y$}](gt) {\includegraphics[height=1.2cm ]{Figures/27_GT.png}};
    \node[square, text width = 1.5cm, align=center, right = 0.75cm of gt, name=adv](adv) {\footnotesize{Weighted} \large{$\mathcal{L}_{ce}$}};



    \draw[-latex] (bet_map.south) to node[above,rotate=26, yshift=-3, xshift=-10] {weights} (adv);
    % \draw[-latex] (pred) to  node[above,rotate=0] {} (adv);
    \path [draw=black, -latex] 
            ([xshift=0cm]pred.south east) to node[below,rotate=20] {} ([xshift=0.2cm]adv.north west);
    \draw[-latex] (gt) to node[above,rotate=0] {} (adv);
    \draw[-latex] (x) to node[above,rotate=0] {} (enc1);
    \draw[-latex] (enc1) to node[above,rotate=0] {} (enc2);
    \draw[-latex] (enc2) to node[above,rotate=0] {} (enc3);
    \draw[-latex] (enc3) to node[above,rotate=0] {} (enc4);
    \draw[-latex] (enc4) to node[above,rotate=0] {} (dec1);
    \draw[-latex] (dec1) to node[above,rotate=0] {} (dec2);
    \draw[-latex] (dec2) to node[above,rotate=0] {} (dec3);
    \draw[-latex] (dec3) to node[above,rotate=0] {} (pred);
    
    \draw[-latex] (pred) to node[above,rotate=0] {} (enc2_1);
    \draw[-latex] (enc2_1) to node[above,rotate=0] {} (enc2_2);
    \draw[-latex] (enc2_2) to node[above,rotate=0] {} (enc2_3);
    \draw[-latex] (enc2_3) to node[above,rotate=0] {} (enc2_4);
    \draw[-latex] (enc2_4) to node[above,rotate=0] {} (dec2_1);
    \draw[-latex] (dec2_1) to node[above,rotate=0] {} (dec2_2);
    \draw[-latex] (dec2_2) to node[above,rotate=0] {} (dec2_3);
    \draw[-latex] (dec2_3) to node[above,rotate=0] {} (bet_map);
    



    % \draw[-latex] () to[bend left=10] node[above,rotate=0] {} (enc2_1);
    % % \draw[-latex] (seg) to [bend left=10] node[above,rotate=0] {} (pred);
    % % \draw[-latex] (pred) to[bend left=10] node[above,rotate=0] {} (gam);
    % % \draw[-latex] (pred) to[bend left=10] node[above,rotate=0] {} (ce);
    % % \draw[-latex] (gt) to[bend left=10] node[above,rotate=0] {} (ce);
    % % \draw[-latex] (gam) to[bend left=10] node[above,rotate=0] {} (inv);
    % % \draw[-latex] (inv) to[bend left=10] node[above,rotate=0] {} (mult);
    % % \draw[-latex] (ce) to[bend left=10] node[above,rotate=0] {} (mult);
    % % \draw[-latex] (mult) to[bend left=10] node[above,rotate=0] {} (adv);
    % % % \draw[-latex] (soft) to[bend left=30] node[above,rotate=0] {$\tilde{s}$} (gam);
    % % % \draw[-latex] (gam) to[bend left=30] node[above] {$\hat{b}$} (loss);
    % % % \draw[-latex] (arg) to node[above,rotate=0] {} (mult);
    % % % \draw[-latex] (mult) to node[above,rotate=-90] {} (plus);
    
    % \draw[dashed, -latex, red] (adv.south east) to[out=0, in = 20] node[below,rotate=0] {} (pred.north east);

    
    \path [draw=red, -latex, dashed] 
            ([yshift=-.2cm]adv.north east) to node[below,rotate=20] {\color{red}{B}} ([xshift=.4cm]bet_map.south);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]bet_map.west) to node[above,rotate=0] {} ([yshift=.15cm]dec2_3.east);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]dec2_3.west) to node[above,rotate=0] {} ([yshift=.15cm]dec2_2.east);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]dec2_2.west) to node[above,rotate=0] {} ([yshift=.15cm]dec2_1.east);
\color{red}{    }\path [draw=red, -latex, dashed] 
            ([yshift=.15cm]dec2_1.west) to node[above,rotate=0] {} ([yshift=.15cm]enc2_4.east);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]enc2_4.west) to node[above,rotate=0] {} ([yshift=.15cm]enc2_3.east);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]enc2_3.west) to node[above,rotate=0] {} ([yshift=.15cm]enc2_2.east);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]enc2_2.west) to node[above,rotate=0] {} ([yshift=.15cm]enc2_1.east);
    \path [draw=red, -latex, dashed] 
            ([yshift=.15cm]enc2_1.west) to node[above,rotate=0] {} ([yshift=.15cm]pred.east);
    % \draw[-latex] (bet_map.south) to node[above,rotate=20, yshift=-3, xshift=-10] {weights} (adv);
    % \draw[dashed, -latex, red] (bet_map.north east) to[bend right=40] node[below,rotate=0] {} (pred.north east);
    % \draw[-latex, red] (dec2_3.north) to[bend right=50] node[below,rotate=0] {} (dec2_2.north);
    % \draw[-latex, red] (dec2_2.north) to[bend right=50] node[below,rotate=0] {} (dec2_1.north);
    % \draw[-latex, red] (dec2_1.north) to[bend right=50] node[below,rotate=0] {} (enc2_4.north);
    % \draw[-latex, red] (enc2_4.north) to[bend right=50] node[below,rotate=0] {} (enc2_3.north);
    % \draw[-latex, red] (enc2_3.north) to[bend right=50] node[below,rotate=0] {} (enc2_2.north);
    % \draw[-latex, red] (enc2_2.north) to[bend right=50] node[below,rotate=0] {} (enc2_1.north);
    % \draw[-latex, red] (enc2_1.north) to[bend right=50] node[below,rotate=0] {} (pred.north east);
    % \draw[-latex, red] (pred.north west) to[bend right=50] node[below,rotate=0] {} (dec3.north);
    % \draw[-latex, red] (dec3.north) to[bend right=50] node[below,rotate=0] {} (dec2.north);
    % \draw[-latex, red] (dec2.north) to[bend right=50] node[below,rotate=0] {} (dec1.north);
    % \draw[-latex, red] (dec1.north) to[bend right=50] node[below,rotate=0] {} (enc4.north);
    % \draw[-latex, red] (enc4.north) to[bend right=50] node[below,rotate=0] {} (enc3.north);
    % \draw[-latex, red] (enc3.north) to[bend right=50] node[below,rotate=0] {} (enc2.north);
    % \draw[-latex, red] (enc2.north) to[bend right=50] node[below,rotate=0] {} (enc1.north);
    % % \draw[-latex, red] (mult) to[bend left=10] node[below,rotate=0] {} (inv);
    % % \draw[-latex, red] (inv) to[bend left=10] node[below,rotate=0] {} (gam);
    % % \draw[-latex, red] (gam) to[bend left=10] node[below,rotate=0] {} (pred);
    % % \draw[-latex, red] (pred) to[bend left=10] node[below,rotate=0] {} (seg);
    
    % \draw[-latex, blue] (adv) to[bend left=5] node[above,rotate=0] {} (pred);
    \path [draw=red, -latex, dashed] 
            ([yshift=-.0cm]adv.north west) to node[xshift=0.cm, yshift=-0.0cm, below,rotate=-0] {\color{red}{A}} ([xshift=-0.2cm]pred.south east);
    
    % \draw[-latex, blue] (pred.south west) to[bend left=50] node[above,rotate=0] {} (dec3.south);
    % \draw[-latex, blue] (dec3.south) to[bend left=50] node[above,rotate=0] {} (dec2.south);
    % \draw[-latex, blue] (dec2.south) to[bend left=50] node[above,rotate=0] {} (dec1.south);
    % \draw[-latex, blue] (dec1.south) to[bend left=50] node[above,rotate=0] {} (enc4.south);
    % \draw[-latex, blue] (enc4.south) to[bend left=50] node[above,rotate=0] {} (enc3.south);
    % \draw[-latex, blue] (enc3.south) to[bend left=50] node[above,rotate=0] {} (enc2.south);
    % \draw[-latex, blue] (enc2.south) to[bend left=50] node[above,rotate=0] {} (enc1.south);
 
\end{tikzpicture}
\caption{An overview of gambling adversarial networks. The solid black arrows indicate the forward pass. The red dashed arrows represent the two gradient flows of the weighted cross-entropy loss. Gradient flow A provides pixel-level feedback independent of other pixel predictions. Gradient flow B, going through the gambler network, enables feedback reflecting the inter-pixel and structural consistency.} 
\label{fig:adv_loss_expl}
\end{figure*}
